Extensible Technology-Agnostic Runtime Verification

With numerous specialised technologies available to industry, it has become increasingly frequent for computer systems to be composed of heterogeneous components built over, and using, different technologies and languages. While this enables developers to use the appropriate technologies for specific contexts, it becomes more challenging to ensure the correctness of the overall system. In this paper we propose a framework to enable extensible technology agnostic runtime verification and we present an extension of polyLarva, a runtime-verification tool able to handle the monitoring of heterogeneous-component systems. The approach is then applied to a case study of a component-based artefact using different technologies, namely C and Java.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v{n}: \\
Formal Engineering Approaches to Software Components \\
and Architectures 2013 (FESCA'13)\\
EPTCS 108, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.108.1}{10.4204/EPTCS.108.1}}
\pdfoutput=1

